Using ACL2 To Teach Students About Software Testing

We report on our experience using ACL2 in the classroom to teach students about software testing. The course COSC2300 at the University of Wyoming is a mostly traditional Discrete Mathematics course, but with a clear focus on computer science applications. For instance, the section on logic and proofs is motivated by the desire to write proofs about computer software. We emphasize that the importance of software correctness falls along a spectrum with casual programs on one end and mission-critical ones on the other. Corresponding to this spectrum is a variety of tools, ranging from unit tests, randomized testing of properties, and even formal proofs. In this paper, we describe one of the major activities, in which students use the ACL2 Sedan's counter-example generation facility to investigate properties of various existing checksum algorithms used in error detection. Students are challenged to state the relevant properties correctly, so that the counter-example generation tool is used effectively in all cases, and ACL2 can find formal proofs automatically in some of those.

==> eptcsdata.tex <==
\providecommand{\firstpage}{19}
\providecommand{\publicationstatus}{Rob Sumners, Cuong Chau (Eds.): 17th ACL2 Workshop (ACL2 2022)\\
EPTCS 359, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.359.4}{10.4204/EPTCS.359.4}}
\pdfoutput=1

